RoboBERT: An End-to-end Multimodal Robotic Manipulation Model

Embodied intelligence seamlessly integrates vision, language, and action.~However, most multimodal robotic models rely on massive fine-tuning, incurring high time and hardware costs.~To address this, we introduce RoboBERT, an end-to-end multimodal manipulation model built around a novel two-stage training paradigm.~In the first stage, we freeze most of the vision encoder and train with a single "standard" instruction phrasing, allowing the model to focus on stable policy learning via a CNN-based diffusion policy.~In the second stage, we unfreeze all modules and inject diverse natural language variants, rapidly aligning varied instructions to the already-learned policy without destabilizing performance.~We further employ systematic data augmentations to enhance robustness against visual perturbations.~Without relying on auxiliary datasets, RoboBERT achieves new state-of-the-art (SOTA) mean episode lengths of 4.52 on the CALVIN ABCD-D benchmark and 3.79 on the ABC-D benchmark using only language-labeled expert demonstrations and a comparatively lightweight architecture.Real-robot trials on a 6-DOF manipulator confirm higher success rates than comparable methods trained on identical data.These results demonstrate that our data-augmentation-enhanced two-stage training paradigm delivers efficient, scalable, and broadly applicable performance for multimodal robotic systems.

==> Comparison_of_Different_Augmentation.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}llcccccc@{}}
\toprule
\textbf{Augmentation} & \textbf{Avg. Length} & \textbf{Increment} \\ 
\midrule
No Augmentation & $3.00\pm0.02$ & $+0.00$ \\
Salt-and-Pepper & $3.22\pm0.03$	& $+0.22$ \\
Affine Transformation & $2.75\pm0.03$ & $-0.25$ \\
Color Jitter & $3.65\pm0.02$	& $+0.65$ \\
Robotic Mixup & $3.23\pm0.04$	& $+0.23$ \\
Combining All & $3.52\pm0.02$	& $+0.52$ \\
Combining All w/o Aff. & $3.79\pm0.03$	& $+0.79$ \\


\bottomrule
\end{tabular}
\caption{Comparison of Different Augmentation}
\label{tab:training_comparison}
\end{table}

==> Comparison_of_Different_Training_Methods.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}llcccccc@{}}
\toprule
\textbf{Training Method} & \textbf{Dataset} & \textbf{Avg. Length} \\ 
\midrule
NL. directly & \(ABCD \rightarrow D\) & $3.39\pm0.05$ \\
Two-stage &\(ABCD \rightarrow D\)	& $4.52\pm0.03$ \\
NL. directly & \(ABC \rightarrow D\) & $1.25\pm0.04$ \\
Two-stage &\(ABC \rightarrow D\)	& $3.79\pm0.03$ \\

\bottomrule
\end{tabular}
\caption{Comparison of Different Training Methods}
\label{tab:training_comparison}
\end{table}

==> preamble.tex <==
%
% --- inline annotations
%
\definecolor{tablecolor}{HTML}{ccf2f5} 
\definecolor{tablecolor2}{HTML}{ffcdb4}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\dd}[2]{$#1#2$} 
\newcommand{\ddbf}[2]{\textbf{$#1 \pm #2$}} 
\newcommand{\sdd}[2]{$#1#2$}
\newcommand{\ddbfblue}[1]{\textbf{\textcolor{blue}{#1}}}
\definecolor{mycolor}{HTML}{BD8DE1}
\definecolor{customblue}{HTML}{D68594}
\usepackage[table]{xcolor}
